Logic-based Clustering and Learning for Time-Series Data

To effectively analyze and design cyberphysical systems (CPS), designers today have to combat the data deluge problem, i.e., the burden of processing intractably large amounts of data produced by complex models and experiments. In this work, we utilize monotonic Parametric Signal Temporal Logic (PSTL) to design features for unsupervised classification of time series data. This enables using off-the-shelf machine learning tools to automatically cluster similar traces with respect to a given PSTL formula. We demonstrate how this technique produces interpretable formulas that are amenable to analysis and understanding using a few representative examples. We illustrate this with case studies related to automotive engine testing, highway traffic analysis, and auto-grading massively open online courses.

==> auditability.tex <==
\section{Auditability/Representative Extraction}

One may argue that the existence of an \STL formula corresponding to
the learnt parameter region, while nice is difficult to interpret for
practicing engineers. Rather, it is often more useful to understand by
example the typical and extremal behaviors in the learnt region.
Because the valuations in a concept are monotonically ordered w.r.t.
satisfaction the traces that project closest to $\val_\bot$ and
$\val_\top$ are natural candidate examples (as well as the trace
closest to the center). In the step detection and overshoot case
studies we will see how one can cognitively interpolate and understand
what traces lie between the edge cases.

In this section we attempt to formalize why observing the extremal
examples of the learned concept yields unreasonable confidence in the
concept. We choose to base this formalism around the notion of a
homotopy lifting property\cite{hatcher2000algebraic}. Specifically, we
seek 2 homotopy liftings: first, a map $\hat{\pi}$ s.t. for the
projection $\pi$ and any curve $\theta(\lambda)$ in $\paramspace$,
$\pi(\hat{\pi}(\theta(\lambda))) = \theta(\lambda)$ and
$\hat{\pi}(\theta)(\lambda)$ is a continuous deformation. This first
lifting enables the cognitive interpolation between any two
valuations. The second lifting requires that there is a lifting of the
continuous deformations between curves in $\paramspace$ to a
continuous deformations of the corresponding homotopies in
$\Traces$. The intuition is that when interpolating between examples
we are finding a continuous deformation in $\Traces$ that projects to
a line in $\paramspace$. One imagines an engineer exploring a
concept by adjusting sliders corresponding to parameter
values within the concept. These adjustments correspond to a path
in $\paramspace$ and finding an example that projects to that point
would correspond to the homotopy lifting. We refer to the engineer's
ability to sensibly/systematically explore the concept as ``human
auditability''. The existence of such liftings would imply that one can
simply examine the extremal cases and be confident the there are no
``holes'' or discontinuities in your cognitive interpolation between points.
\footnote{In addition to helping with human auditability, one might
  consider using the learnt homotopies as an environment abstraction
  for model checking/falsification.}


\begin{figure}[htbp]
  \centering
  \includesvg[svgpath = imgs/, height=2in]{higher_homotopy}
  \caption{Illustrates 2 paths in parameter space being mapped to a
    homotopies in the signal space. On the right we give an explicit
    sampling of a lifting of the diagonal in the spike template.
    \label{fig:spike_interp}
  }
\end{figure}

\begin{example}
Consider again the spike template $\f_{h, w}$,
\ref{spike_to_zero} restricted again to $\Traces_{spike}$. Further,
let $\f_B$ encode the bounding box. Define $\psi \triangleq \f \wedge
\f_B$. Notice that $\psi$ is identical in behavior as $\f_{h,w}$, but
is bound to the extracted parameter region.  Observe that any curve
between any two parameters in the bounding box can be lifted to a
homotopy in the signal space s.t.  there exists a projection map $\pi
\in \Pi_\psi$ back to the line.  Namely, fix $\pi$ us lexicographic
order $h \lexOrder w$ and take any curve in the parameter space
$\theta : [0, 1] \rightarrow \paramspace$.  Recalling that the
lexicographic ordering exactly recovers $w$ and $h$, a valid homotopy
lifting of $\theta(\lambda)$ into $X$ is:
\begin{equation}
  g(t, \lambda) = f(\theta(\lambda), t)
\end{equation}

Recall that without our lifting condition, any 2 continuous curves
between two points in the parameter space are in the same homotopy
class (inherited from $\mathbb{R}^{|\theta|}$). Also notice that there
are no curves in the bounding hyperbox that cannot be lifted. Thus, we
can continuously deform both the curve in the parameter space and the
homotopy in $\Traces_{spike}$.
\end{example}

\noindent We conjecture the following to be true for any learnt
concept, and leave them open.
\begin{compactenum}
\item Between any two points in a comparably convex concept, there is a
  monotonically increasing curve that can be lifted to the signal space.
\item Between any 2 monotonic curves in the parameter region, there
  exists a homotopy between them (in the set on monotonic curves) that
  satisfies the lifting property.
\item Between all the Manhattan Paths and the box diagonal in the
  parameter space, there exists a homotopy that can be lifted.
\end{compactenum}


==> environments.tex <==
\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}{Proposition}[section]
\newtheorem{lemma}{Lemma}[section]
\newtheorem{hypothesis}{Hypothesis}[section]
\newtheorem{conjecture}{Conjecture}[section]
\newtheorem{corollary}{Corollary}[section]

\newtheorem{definition}{Definition}[section]
\newdef{example}{Example}
\newdef{remark}{Remark}


==> fuzz_base_value.tex <==
\begin{tabular}{lrr}
\toprule
{} &          l &          u \\
label &            &            \\
\midrule
0     &       0.00 &       0.00 \\
2     &       0.46 &       0.44 \\
3     &       0.12 &       0.07 \\
\bottomrule
\end{tabular}


==> fuzz_polarities_value.tex <==
\begin{tabular}{lrr}
\toprule
{} &    l\_width &    u\_width \\
label &            &            \\
\midrule
0     &       0.12 &       0.98 \\
2     &       0.54 &       0.40 \\
3     &       0.27 &       0.93 \\
\bottomrule
\end{tabular}


==> gradlew <==
#!/usr/bin/env bash

##############################################################################
##
##  Gradle start up script for UN*X
##
##############################################################################

# Attempt to set APP_HOME
# Resolve links: $0 may be a link
PRG="$0"
# Need this for relative symlinks.
while [ -h "$PRG" ] ; do
    ls=`ls -ld "$PRG"`
    link=`expr "$ls" : '.*-> \(.*\)$'`
    if expr "$link" : '/.*' > /dev/null; then
        PRG="$link"
    else
        PRG=`dirname "$PRG"`"/$link"
    fi
done
SAVED="`pwd`"
cd "`dirname \"$PRG\"`/" >/dev/null
APP_HOME="`pwd -P`"
cd "$SAVED" >/dev/null

APP_NAME="Gradle"
APP_BASE_NAME=`basename "$0"`

# Add default JVM options here. You can also use JAVA_OPTS and GRADLE_OPTS to pass JVM options to this script.
DEFAULT_JVM_OPTS=""

# Use the maximum available, or set MAX_FD != -1 to use that value.
MAX_FD="maximum"

warn ( ) {
    echo "$*"
}

die ( ) {
    echo
    echo "$*"
    echo
    exit 1
}

# OS specific support (must be 'true' or 'false').
cygwin=false
msys=false
darwin=false
nonstop=false
case "`uname`" in
  CYGWIN* )
    cygwin=true
    ;;
  Darwin* )
    darwin=true
    ;;
  MINGW* )
    msys=true
    ;;
  NONSTOP* )
    nonstop=true
    ;;
esac

CLASSPATH=$APP_HOME/gradle/wrapper/gradle-wrapper.jar

# Determine the Java command to use to start the JVM.
if [ -n "$JAVA_HOME" ] ; then
    if [ -x "$JAVA_HOME/jre/sh/java" ] ; then
        # IBM's JDK on AIX uses strange locations for the executables
        JAVACMD="$JAVA_HOME/jre/sh/java"
    else
        JAVACMD="$JAVA_HOME/bin/java"
    fi
    if [ ! -x "$JAVACMD" ] ; then
        die "ERROR: JAVA_HOME is set to an invalid directory: $JAVA_HOME

Please set the JAVA_HOME variable in your environment to match the
location of your Java installation."
    fi
else
    JAVACMD="java"
    which java >/dev/null 2>&1 || die "ERROR: JAVA_HOME is not set and no 'java' command could be found in your PATH.

Please set the JAVA_HOME variable in your environment to match the
location of your Java installation."
fi

# Increase the maximum file descriptors if we can.
if [ "$cygwin" = "false" -a "$darwin" = "false" -a "$nonstop" = "false" ] ; then
    MAX_FD_LIMIT=`ulimit -H -n`
    if [ $? -eq 0 ] ; then
        if [ "$MAX_FD" = "maximum" -o "$MAX_FD" = "max" ] ; then
            MAX_FD="$MAX_FD_LIMIT"
        fi
        ulimit -n $MAX_FD
        if [ $? -ne 0 ] ; then
            warn "Could not set maximum file descriptor limit: $MAX_FD"
        fi
    else
        warn "Could not query maximum file descriptor limit: $MAX_FD_LIMIT"
    fi
fi

# For Darwin, add options to specify how the application appears in the dock
if $darwin; then
    GRADLE_OPTS="$GRADLE_OPTS \"-Xdock:name=$APP_NAME\" \"-Xdock:icon=$APP_HOME/media/gradle.icns\""
fi

# For Cygwin, switch paths to Windows format before running java
if $cygwin ; then
    APP_HOME=`cygpath --path --mixed "$APP_HOME"`
    CLASSPATH=`cygpath --path --mixed "$CLASSPATH"`
    JAVACMD=`cygpath --unix "$JAVACMD"`

    # We build the pattern for arguments to be converted via cygpath
    ROOTDIRSRAW=`find -L / -maxdepth 1 -mindepth 1 -type d 2>/dev/null`
    SEP=""
    for dir in $ROOTDIRSRAW ; do
        ROOTDIRS="$ROOTDIRS$SEP$dir"
        SEP="|"
    done
    OURCYGPATTERN="(^($ROOTDIRS))"
    # Add a user-defined pattern to the cygpath arguments
    if [ "$GRADLE_CYGPATTERN" != "" ] ; then
        OURCYGPATTERN="$OURCYGPATTERN|($GRADLE_CYGPATTERN)"
    fi
    # Now convert the arguments - kludge to limit ourselves to /bin/sh
    i=0
    for arg in "$@" ; do
        CHECK=`echo "$arg"|egrep -c "$OURCYGPATTERN" -`
        CHECK2=`echo "$arg"|egrep -c "^-"`                                 ### Determine if an option

        if [ $CHECK -ne 0 ] && [ $CHECK2 -eq 0 ] ; then                    ### Added a condition
            eval `echo args$i`=`cygpath --path --ignore --mixed "$arg"`
        else
            eval `echo args$i`="\"$arg\""
        fi
        i=$((i+1))
    done
    case $i in
        (0) set -- ;;
        (1) set -- "$args0" ;;
        (2) set -- "$args0" "$args1" ;;
        (3) set -- "$args0" "$args1" "$args2" ;;
        (4) set -- "$args0" "$args1" "$args2" "$args3" ;;
        (5) set -- "$args0" "$args1" "$args2" "$args3" "$args4" ;;
        (6) set -- "$args0" "$args1" "$args2" "$args3" "$args4" "$args5" ;;
        (7) set -- "$args0" "$args1" "$args2" "$args3" "$args4" "$args5" "$args6" ;;
        (8) set -- "$args0" "$args1" "$args2" "$args3" "$args4" "$args5" "$args6" "$args7" ;;
        (9) set -- "$args0" "$args1" "$args2" "$args3" "$args4" "$args5" "$args6" "$args7" "$args8" ;;
    esac
fi

# Split up the JVM_OPTS And GRADLE_OPTS values into an array, following the shell quoting and substitution rules
function splitJvmOpts() {
    JVM_OPTS=("$@")
}
eval splitJvmOpts $DEFAULT_JVM_OPTS $JAVA_OPTS $GRADLE_OPTS
JVM_OPTS[${#JVM_OPTS[*]}]="-Dorg.gradle.appname=$APP_BASE_NAME"

exec "$JAVACMD" "${JVM_OPTS[@]}" -classpath "$CLASSPATH" org.gradle.wrapper.GradleWrapperMain "$@"


==> imgs/spike_cluster_illustration.tex <==
\begin{figure}[t]
\begin{minipage}[c]{0.30\textwidth}
\begin{tikzpicture}[>=stealth']
 
   \draw[thick,->] (-0.1, 0) -- (4.8,0) node[pos = 0.98, above] {$w$}; 
   \draw[thick,->] (0, -0.1) -- (0,3.8) node[pos=0.95, right] {$h$};
  

  %first cluster
  \draw[thick, densely dotted] (0.2, 0.2) rectangle (1.2,0.8);

  % second cluster
  \draw[thick, densely dotted] (2.2, 0.5) rectangle (2.8,1.5);
  % third cluster
  \def \x {0.8}
  \def \y {1.2}
  \def \xt{1.4}
  \def \yt{3}

  \draw[thick, densely dotted] (\x, \y) node[below, left](l1) {(10)}  node[right= {\xt-\x} of l1]{(00)} rectangle (\xt,\yt) node[above, right] (l2) {(01)} node[above = 1.25 of l1]{(11)} ;
  \foreach \Point in { (\x, \y), (\xt, \y), (\x, \yt), (
  \xt,\yt)} {
	\node at \Point {\textbullet};
  }
  \draw[->] ({(\x+\xt)/2}, \yt) -- ({(\x+\xt)/2}, {\yt+0.3});
  \draw[->] (\x, {(\y+\yt)/2}) -- ({\x-0.3}, {(\y+\yt)/2});
	
  \foreach \Cross in {(0.22, 0.23), (0.4, 0.7), (0.5, 0.35),
  (0.75,0.45), (1.15,0.55), (1.1,0.3), (0.6,0.4), (0.7,0.65),  
  (2.3, 0.55), (2.5, 1.1), (2.6, 0.6), (2.5, 1.42), (2.75, 1.2),
  ({\x+0.05}, {\yt-0.8}), ({\x+0.5}, {\y+2}), ({\x+0.23}, {\yt-0.05}), ({\xt-0.2}, {\y+0.4}), ({\xt-0.3}, {\y+1.5}),
  ({\x+0.3}, {\y+0.4}), ({\x+0.15}, {\y+0.8}), ({\x+0.55}, {\y+1.2}) , ({\x+0.27}, {\y+0.98}), ({\x+0.15}, {\y+0.05})
  }
  {
	\node at \Cross {x};
  }
\newcommand{\exampleTraj}[5]{%
% #1 #2 position shift for the corner of the example
% #3 #4 width and length of spike_illustration
\def \w {#3}
\begin{scope}[xshift=#1,yshift=#2]
\draw [semithick] (0, 0) rectangle(1.2, 0.8);
% draw the trajectory line
\draw [thick] (0.1, 0.1) -- ({0.6-\w/2}, 0.1) 
-- (0.6, #4) -- ({0.6+\w/2}, 0.1) 
-- (1.1, 0.1);
\end{scope}
}  

\exampleTraj{1.9cm}{1.9cm}{0.2}{0.7}{e1}
% \exampleTraj{4cm}{2cm}{0.3}{0.5}{e2}
\exampleTraj{3.2cm}{1.2cm}{0.7}{0.4}{e3}
\exampleTraj{3.2cm}{0.1cm}{0.1}{0.15}{e4}

\draw[->, densely dotted] ({\x+0.23}, {\yt-0.05}) -- (1.9, 2.2);
\draw[->, densely dotted] (2.5, 1.42) -- (3.2, 1.42);
\draw[->, densely dotted] (0.22, 0.23) -- (3.2, 0.23);

\node[align = center] at (4.1,3.2) {$sgn(h) = -$ \\ $sgn(w) = +$};  
\end{tikzpicture}
\end{minipage} \hfill
\begin{minipage}[l]{0.15 \textwidth}
\caption{Illustration hypothetical three cluster distributions and examples of spike instances.}
\label{fig:spike_illustration}
\end{minipage}
\end{figure}

